Classification with Rejection Based on Cost-sensitive Classification

The goal of classification with rejection is to avoid risky misclassification in error-critical applications such as medical diagnosis and product inspection. In this paper, based on the relationship between classification with rejection and cost-sensitive classification, we propose a novel method of classification with rejection by learning an ensemble of cost-sensitive classifiers, which satisfies all the following properties: (i) it can avoid estimating class-posterior probabilities, resulting in improved classification accuracy, (ii) it allows a flexible choice of losses including non-convex ones, (iii) it does not require complicated modifications when using different losses, (iv) it is applicable to both binary and multiclass cases, and (v) it is theoretically justifiable for any classification-calibrated loss. Experimental results demonstrate the usefulness of our proposed approach in clean-labeled, noisy-labeled, and positive-unlabeled classification.

==> tab_results.tex <==
\begin{table*}[t]
\centering
\resizebox{.95\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
Dataset & $c$ 
& SCE & DEFER & OVA-squared& CS-squared& CS-hinge & CS-sigmoid \\
\midrule
\multirow{7}{*}{Gisette}
& 0.10
& $2.40(0.10)$ & $5.41(0.12)$ & $6.06(0.21)$ 
& $5.83(0.25)$ & $2.41(0.08)$ & $\mathbf{2.27(0.08)}$ \\
& 0.15
& $2.70(0.14)$ & $6.56(0.15)$ & $7.87(0.30)$ 
& $7.34(0.25)$ & $\mathbf{2.64(0.13)}$ & $\mathbf{2.58(0.05)}$ \\
& 0.20
& $2.90(0.12)$ & $7.64(0.14)$ & $9.23(0.22)$ 
& $8.37(0.24)$ & $\mathbf{2.71(0.09)}$ & $\mathbf{2.76(0.06)}$ \\
& 0.25
& $3.26(0.12)$ & $8.74(0.16)$ & $10.16(0.32)$ 
& $9.12(0.37)$ & $\mathbf{2.90(0.07)}$ & $\mathbf{2.95(0.06)}$ \\
& 0.30
& $3.41(0.13)$ & $9.80(0.22)$ & $10.84(0.37)$ 
& $10.13(0.52)$ & $3.21(0.12)$ & $\mathbf{3.08(0.08)}$ \\
& 0.35
& $3.55(0.10)$ & $10.75(0.23)$ & $11.41(0.33)$ 
& $10.80(0.32)$ & $\mathbf{3.32(0.13)}$ & $\mathbf{3.26(0.04)}$ \\
& 0.40
& $3.73(0.16)$ & $11.51(0.20)$ & $11.62(0.45)$ 
& $11.16(0.37)$ & $3.55(0.14)$ & $\mathbf{3.35(0.06)}$ \\
\midrule
\multirow{7}{*}{Phishing}
& 0.10
& $4.30(0.26)$ & $5.48(0.01)$ & $5.67(0.02)$ 
& $4.56(0.05)$ & $\mathbf{3.48(0.03)}$ & $4.25(0.12)$ \\
& 0.15
& $5.38(0.29)$ & $7.58(0.04)$ & $7.18(0.02)$ 
& $5.43(0.03)$ & $\mathbf{4.84(0.03)}$ & $5.30(0.07)$ \\
& 0.20
& $6.51(0.22)$ & $9.30(0.03)$ & $8.06(0.04)$ 
& $6.37(0.02)$ & $\mathbf{5.75(0.06)}$ & $6.28(0.10)$ \\
& 0.25
& $7.52(0.29)$ & $10.61(0.03)$ & $8.22(0.03)$ 
& $7.19(0.03)$ & $\mathbf{6.09(0.07)}$ & $7.01(0.06)$ \\
& 0.30
& $8.17(0.31)$ & $11.34(0.04)$ & $8.40(0.02)$ 
& $7.47(0.03)$ & $\mathbf{6.55(0.07)}$ & $7.60(0.18)$ \\
& 0.35
& $8.77(0.42)$ & $11.72(0.06)$ & $8.09(0.04)$ 
& $7.71(0.03)$ & $\mathbf{7.09(0.06)}$ & $7.88(0.16)$ \\
& 0.40
& $9.04(0.61)$ & $12.08(0.04)$ & $8.11(0.03)$ 
& $7.81(0.03)$ & $\mathbf{7.21(0.05)}$ & $8.15(0.10)$ \\
\midrule
\multirow{7}{*}{Spambase}
& 0.10
& $5.91(0.21)$ & $6.96(0.06)$ & $7.70(0.01)$ 
& $6.26(0.08)$ & $\mathbf{5.43(0.07)}$ & $6.65(0.22)$ \\
& 0.15
& $7.24(0.29)$ & $8.83(0.10)$ & $10.13(0.03)$ 
& $8.15(0.10)$ & $\mathbf{6.82(0.13)}$ & $8.14(0.22)$ \\
& 0.20
& $8.80(0.51)$ & $10.31(0.15)$ & $11.95(0.17)$ 
& $9.50(0.13)$ & $\mathbf{7.66(0.12)}$ & $8.75(0.29)$ \\
& 0.25
& $9.81(0.40)$ & $11.26(0.27)$ & $12.54(0.02)$ 
& $9.95(0.07)$ & $\mathbf{8.12(0.11)}$ & $8.99(0.14)$ \\
& 0.30
& $10.84(0.68)$ & $11.86(0.22)$ & $12.56(0.06)$ 
& $10.17(0.13)$ & $\mathbf{8.55(0.13)}$ & $9.07(0.12)$ \\
& 0.35
& $11.79(0.78)$ & $12.18(0.21)$ & $12.16(0.06)$ 
& $10.63(0.09)$ & $\mathbf{8.86(0.12)}$ & $9.34(0.19)$ \\
& 0.40
& $12.43(0.92)$ & $11.93(0.22)$ & $11.72(0.03)$ 
& $11.24(0.07)$ & $\mathbf{8.95(0.10)}$ & $9.62(0.20)$ \\
\midrule
\multirow{7}{*}{Subj}
& 0.10
& $6.88(0.19)$ & $6.98(0.03)$ & $7.27(0.02)$ 
& $7.19(0.02)$ & $\mathbf{6.35(0.05)}$ & $8.08(0.06)$ \\
& 0.15
& $8.52(0.23)$ & $9.56(0.05)$ & $9.87(0.08)$ 
& $8.59(0.04)$ & $\mathbf{7.92(0.06)}$ & $9.09(0.05)$ \\
& 0.20
& $9.98(0.17)$ & $11.71(0.05)$ & $11.44(0.06)$ 
& $9.60(0.05)$ & $\mathbf{9.29(0.05)}$ & $9.88(0.07)$ \\
& 0.25
& $10.96(0.23)$ & $13.41(0.05)$ & $12.14(0.06)$ 
& $10.31(0.07)$ & $\mathbf{10.25(0.06)}$ & $10.57(0.07)$ \\
& 0.30
& $11.92(0.21)$ & $14.87(0.07)$ & $12.55(0.07)$ 
& $11.05(0.04)$ & $\mathbf{10.78(0.07)}$ & $11.09(0.05)$ \\
& 0.35
& $13.05(0.20)$ & $15.96(0.05)$ & $12.46(0.04)$ 
& $11.52(0.06)$ & $\mathbf{11.28(0.06)}$ & $11.37(0.06)$ \\
& 0.40
& $14.01(0.28)$ & $16.38(0.09)$ & $12.43(0.04)$ 
& $11.69(0.10)$ & $\mathbf{11.51(0.07)}$ & $11.60(0.06)$ \\
\midrule
\multirow{7}{*}{Twonorm}
& 0.10
& $1.45(0.09)$ & $5.16(0.05)$ & $5.10(0.02)$ 
& $1.88(0.04)$ & $\mathbf{1.36(0.07)}$ & $1.43(0.06)$ \\
& 0.15
& $1.89(0.12)$ & $7.20(0.08)$ & $6.07(0.02)$ 
& $1.73(0.03)$ & $\mathbf{1.59(0.05)}$ & $\mathbf{1.58(0.09)}$ \\
& 0.20
& $2.23(0.19)$ & $8.73(0.09)$ & $6.37(0.02)$ 
& $1.84(0.02)$ & $1.80(0.06)$ & $\mathbf{1.74(0.07)}$ \\
& 0.25
& $2.55(0.16)$ & $9.96(0.06)$ & $5.79(0.02)$ 
& $\mathbf{1.87(0.02)}$ & $1.99(0.05)$ & $1.92(0.04)$ \\
& 0.30
& $2.84(0.18)$ & $10.81(0.11)$ & $5.01(0.01)$ 
& $\mathbf{1.97(0.01)}$ & $2.09(0.04)$ & $2.05(0.06)$ \\
& 0.35
& $3.12(0.17)$ & $11.16(0.08)$ & $3.90(0.02)$ 
& $\mathbf{2.12(0.02)}$ & $2.22(0.05)$ & $2.22(0.08)$ \\
& 0.40
& $3.39(0.35)$ & $11.17(0.06)$ & $3.20(0.02)$ 
& $\mathbf{2.19(0.01)}$ & $2.27(0.10)$ & $2.31(0.08)$ \\
\midrule
\multirow{7}{*}{MNIST}
& 0.10
& $0.85(0.08)$ & $3.27(0.64)$ & $1.82(0.24)$ 
& $0.62(0.03)$ & $\mathbf{0.41(0.02)}$ & $1.31(1.03)$ \\
& 0.15
& $0.82(0.09)$ & $3.94(0.51)$ & $1.44(0.13)$ 
& $0.68(0.04)$ & $\mathbf{0.48(0.03)}$ & $1.71(1.09)$ \\
& 0.20
& $0.83(0.07)$ & $4.90(0.89)$ & $1.26(0.08)$ 
& $0.69(0.04)$ & $\mathbf{0.54(0.04)}$ & $1.15(0.81)$ \\
& 0.25
& $0.88(0.12)$ & $4.74(0.89)$ & $1.10(0.06)$ 
& $0.76(0.04)$ & $\mathbf{0.62(0.04)}$ & $0.91(0.09)$ \\
& 0.30
& $0.84(0.07)$ & $5.10(0.80)$ & $0.96(0.05)$ 
& $0.84(0.05)$ & $\mathbf{0.72(0.05)}$ & $1.67(1.17)$ \\
& 0.35
& $\mathbf{0.86(0.08)}$ & $4.81(0.83)$ & $0.90(0.04)$ 
& $0.96(0.07)$ & $\mathbf{0.86(0.06)}$ & $1.61(1.05)$ \\
& 0.40
& $\mathbf{0.83(0.09)}$ & $4.02(0.50)$ & $\mathbf{0.79(0.04)}$ 
& $1.06(0.04)$ & $0.97(0.10)$ & $1.47(0.20)$ \\
\midrule
\multirow{7}{*}{Fashion-MNIST}
& 0.10
& $8.49(0.16)$ & $5.76(0.31)$ & $\mathbf{4.62(0.19)}$ 
& $4.88(0.15)$ & $5.02(0.16)$ & $6.64(1.22)$ \\
& 0.15
& $8.37(0.17)$ & $7.86(0.76)$ & $\mathbf{5.59(0.09)}$ 
& $\mathbf{5.64(0.12)}$ & $\mathbf{5.58(0.12)}$ & $7.58(1.00)$ \\
& 0.20
& $8.37(0.18)$ & $9.25(0.68)$ & $6.27(0.16)$ 
& $\mathbf{6.13(0.09)}$ & $\mathbf{6.05(0.13)}$ & $7.24(0.63)$ \\
& 0.25
& $8.51(0.24)$ & $10.20(0.84)$ & $6.74(0.08)$ 
& $\mathbf{6.61(0.08)}$ & $\mathbf{6.56(0.09)}$ & $7.51(0.71)$ \\
& 0.30
& $8.46(0.14)$ & $11.23(0.91)$ & $\mathbf{7.23(0.22)}$ 
& $7.40(0.11)$ & $\mathbf{7.33(0.17)}$ & $8.25(0.39)$ \\
& 0.35
& $8.51(0.15)$ & $11.71(1.05)$ & $\mathbf{7.52(0.12)}$ 
& $8.34(0.16)$ & $8.00(0.25)$ & $9.65(1.01)$ \\
& 0.40
& $8.43(0.15)$ & $11.94(0.72)$ & $\mathbf{7.87(0.16)}$ 
& $9.89(0.18)$ & $9.12(0.36)$ & $10.70(0.48)$ \\
\midrule
\multirow{7}{*}{KMNIST}
& 0.10
& $5.81(0.23)$ & $5.14(0.20)$ & $4.36(0.35)$ 
& $2.94(0.08)$ & $\mathbf{2.69(0.10)}$ & $3.85(0.74)$ \\
& 0.15
& $5.71(0.23)$ & $7.32(0.47)$ & $5.18(0.22)$ 
& $3.52(0.07)$ & $\mathbf{3.27(0.14)}$ & $4.28(0.40)$ \\
& 0.20
& $5.70(0.24)$ & $8.75(0.40)$ & $5.36(0.20)$ 
& $4.04(0.10)$ & $\mathbf{3.71(0.13)}$ & $5.24(1.25)$ \\
& 0.25
& $5.82(0.16)$ & $10.32(0.67)$ & $5.33(0.27)$ 
& $4.45(0.12)$ & $\mathbf{4.21(0.12)}$ & $6.07(1.08)$ \\
& 0.30
& $5.79(0.22)$ & $11.78(0.96)$ & $5.41(0.20)$ 
& $4.92(0.13)$ & $\mathbf{4.74(0.19)}$ & $6.08(0.75)$ \\
& 0.35
& $5.79(0.24)$ & $12.09(1.02)$ & $\mathbf{5.26(0.18)}$ 
& $5.57(0.20)$ & $\mathbf{5.33(0.20)}$ & $6.84(0.42)$ \\
& 0.40
& $5.69(0.21)$ & $12.15(0.57)$ & $\mathbf{5.42(0.16)}$ 
& $6.11(0.20)$ & $5.90(0.22)$ & $7.73(0.44)$ \\
\bottomrule
\end{tabular}
} % \resizebox
\caption{Mean and standard error of $0\text{-}1\text{-}c$ risk of the clean-labeled setting (rescaled to $0-100$). }
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table*}[t]
\centering
\resizebox{.95\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
Dataset & $c$ 
& SCE & DEFER & OVA-squared& CS-squared& CS-hinge & CS-sigmoid \\
\midrule
\multirow{7}{*}{Gisette}
& 0.10
& $4.84(0.26)$ & $25.83(0.36)$ & $44.53(0.70)$ 
& $8.84(0.61)$ & $3.68(0.22)$ & $\mathbf{3.21(0.21)}$ \\
& 0.15
& $4.59(0.17)$ & $25.27(0.37)$ & $38.78(1.00)$ 
& $8.68(0.85)$ & $3.53(0.24)$ & $\mathbf{2.65(0.08)}$ \\
& 0.20
& $4.39(0.34)$ & $24.83(0.47)$ & $32.95(0.50)$ 
& $8.03(0.53)$ & $3.24(0.22)$ & $\mathbf{2.32(0.10)}$ \\
& 0.25
& $3.90(0.38)$ & $24.29(0.38)$ & $26.86(0.70)$ 
& $7.62(0.97)$ & $3.22(0.28)$ & $\mathbf{1.89(0.18)}$ \\
& 0.30
& $4.00(0.43)$ & $23.60(0.50)$ & $21.43(0.74)$ 
& $7.54(0.80)$ & $3.16(0.33)$ & $\mathbf{1.67(0.15)}$ \\
& 0.35
& $3.72(0.33)$ & $23.17(0.51)$ & $15.81(0.45)$ 
& $7.44(0.86)$ & $3.09(0.28)$ & $\mathbf{1.33(0.12)}$ \\
& 0.40
& $3.34(0.30)$ & $22.37(0.47)$ & $10.82(0.49)$ 
& $7.36(0.64)$ & $3.00(0.16)$ & $\mathbf{1.19(0.14)}$ \\
\midrule
\multirow{7}{*}{Phishing}
& 0.10
& $\mathbf{23.39(3.19)}$ & $53.22(0.14)$ & $55.95(0.19)$ 
& $44.76(0.53)$ & $26.45(0.91)$ & $\mathbf{21.66(1.05)}$ \\
& 0.15
& $21.70(2.53)$ & $49.03(0.26)$ & $46.64(0.14)$ 
& $24.26(0.13)$ & $\mathbf{19.90(0.60)}$ & $\mathbf{19.58(0.82)}$ \\
& 0.20
& $22.35(2.23)$ & $44.31(0.20)$ & $37.15(0.17)$ 
& $14.86(0.10)$ & $\mathbf{13.85(0.51)}$ & $16.69(0.75)$ \\
& 0.25
& $19.71(2.23)$ & $40.10(0.20)$ & $27.02(0.16)$ 
& $\mathbf{8.65(0.11)}$ & $10.18(0.26)$ & $14.07(0.59)$ \\
& 0.30
& $17.32(1.96)$ & $34.55(0.16)$ & $19.11(0.10)$ 
& $\mathbf{4.91(0.03)}$ & $6.87(0.51)$ & $11.23(0.36)$ \\
& 0.35
& $16.25(1.92)$ & $29.71(0.17)$ & $12.17(0.07)$ 
& $\mathbf{3.08(0.04)}$ & $4.33(0.37)$ & $8.40(0.47)$ \\
& 0.40
& $14.12(2.31)$ & $25.34(0.15)$ & $6.31(0.06)$ 
& $\mathbf{1.94(0.04)}$ & $2.42(0.12)$ & $5.69(0.50)$ \\
\midrule
\multirow{7}{*}{Spambase}
& 0.10
& $34.82(3.33)$ & $43.15(1.25)$ & $70.02(0.16)$ 
& $55.56(1.01)$ & $39.17(1.49)$ & $\mathbf{28.39(1.33)}$ \\
& 0.15
& $31.24(3.67)$ & $39.25(1.80)$ & $61.50(0.13)$ 
& $47.38(1.58)$ & $29.13(2.03)$ & $\mathbf{24.31(1.06)}$ \\
& 0.20
& $29.04(4.37)$ & $34.03(0.86)$ & $50.65(1.03)$ 
& $37.14(0.94)$ & $\mathbf{17.54(1.32)}$ & $\mathbf{16.69(0.93)}$ \\
& 0.25
& $26.25(3.16)$ & $29.07(1.26)$ & $39.02(0.15)$ 
& $25.84(0.60)$ & $\mathbf{12.28(0.76)}$ & $\mathbf{12.76(0.55)}$ \\
& 0.30
& $25.66(3.58)$ & $24.32(1.01)$ & $29.51(0.10)$ 
& $19.30(0.47)$ & $\mathbf{9.14(0.44)}$ & $\mathbf{9.32(0.45)}$ \\
& 0.35
& $23.82(3.30)$ & $20.25(0.81)$ & $21.52(0.11)$ 
& $14.47(0.32)$ & $\mathbf{6.63(0.55)}$ & $\mathbf{6.40(0.49)}$ \\
& 0.40
& $21.77(3.28)$ & $15.41(0.87)$ & $13.62(0.17)$ 
& $9.15(0.18)$ & $4.47(0.37)$ & $\mathbf{4.06(0.46)}$ \\
\midrule
\multirow{7}{*}{Subj}
& 0.10
& $29.57(1.85)$ & $58.37(0.36)$ & $66.12(0.31)$ 
& $64.30(0.28)$ & $33.15(0.41)$ & $\mathbf{14.63(0.26)}$ \\
& 0.15
& $27.65(1.58)$ & $54.13(0.29)$ & $57.97(0.55)$ 
& $43.55(0.21)$ & $24.47(0.36)$ & $\mathbf{12.76(0.32)}$ \\
& 0.20
& $25.65(1.50)$ & $50.05(0.14)$ & $48.75(0.20)$ 
& $30.50(0.24)$ & $19.56(0.15)$ & $\mathbf{11.01(0.30)}$ \\
& 0.25
& $24.88(1.46)$ & $45.60(0.19)$ & $39.59(0.26)$ 
& $21.90(0.15)$ & $15.64(0.19)$ & $\mathbf{9.53(0.28)}$ \\
& 0.30
& $21.68(2.34)$ & $41.15(0.23)$ & $30.74(0.19)$ 
& $16.48(0.17)$ & $11.78(0.13)$ & $\mathbf{7.91(0.27)}$ \\
& 0.35
& $21.73(1.70)$ & $36.56(0.27)$ & $22.17(0.12)$ 
& $11.66(0.14)$ & $8.81(0.17)$ & $\mathbf{6.40(0.15)}$ \\
& 0.40
& $20.87(1.28)$ & $31.34(0.27)$ & $14.71(0.14)$ 
& $7.59(0.09)$ & $5.92(0.12)$ & $\mathbf{4.55(0.18)}$ \\
\midrule
\multirow{7}{*}{Twonorm}
& 0.10
& $9.62(1.33)$ & $51.57(0.48)$ & $50.98(0.23)$ 
& $18.15(0.51)$ & $5.69(0.59)$ & $\mathbf{3.84(0.47)}$ \\
& 0.15
& $8.54(1.08)$ & $48.00(0.52)$ & $40.45(0.12)$ 
& $8.99(0.27)$ & $4.69(0.49)$ & $\mathbf{3.98(0.37)}$ \\
& 0.20
& $8.08(1.60)$ & $43.64(0.47)$ & $31.72(0.12)$ 
& $5.62(0.04)$ & $\mathbf{3.82(0.48)}$ & $\mathbf{3.58(0.38)}$ \\
& 0.25
& $7.43(0.96)$ & $39.86(0.24)$ & $22.95(0.06)$ 
& $3.82(0.03)$ & $\mathbf{3.20(0.19)}$ & $\mathbf{3.23(0.34)}$ \\
& 0.30
& $7.21(0.83)$ & $35.96(0.36)$ & $16.34(0.04)$ 
& $\mathbf{2.72(0.03)}$ & $\mathbf{2.63(0.16)}$ & $2.88(0.16)$ \\
& 0.35
& $6.64(0.95)$ & $31.82(0.22)$ & $10.37(0.07)$ 
& $\mathbf{2.00(0.04)}$ & $\mathbf{2.03(0.11)}$ & $2.40(0.28)$ \\
& 0.40
& $6.37(1.19)$ & $27.81(0.16)$ & $6.39(0.05)$ 
& $\mathbf{1.32(0.03)}$ & $1.41(0.12)$ & $1.70(0.14)$ \\
\midrule
\multirow{7}{*}{MNIST}
& 0.10
& $\mathbf{0.00(0.00)}$ & $32.48(6.39)$ & $18.07(2.36)$ 
& $2.38(0.16)$ & $1.32(0.17)$ & $8.75(9.53)$ \\
& 0.15
& $\mathbf{0.00(0.00)}$ & $26.13(3.38)$ & $9.34(0.93)$ 
& $1.64(0.08)$ & $1.27(0.09)$ & $8.38(7.22)$ \\
& 0.20
& $\mathbf{0.00(0.00)}$ & $24.39(4.45)$ & $5.89(0.45)$ 
& $1.37(0.11)$ & $1.30(0.08)$ & $3.75(3.80)$ \\
& 0.25
& $\mathbf{0.00(0.00)}$ & $18.83(3.56)$ & $3.78(0.30)$ 
& $1.36(0.09)$ & $1.31(0.14)$ & $2.02(0.20)$ \\
& 0.30
& $\mathbf{0.00(0.00)}$ & $16.89(2.70)$ & $2.41(0.17)$ 
& $1.39(0.12)$ & $1.40(0.09)$ & $4.09(3.67)$ \\
& 0.35
& $\mathbf{0.00(0.00)}$ & $13.62(2.37)$ & $1.38(0.12)$ 
& $1.59(0.09)$ & $1.62(0.17)$ & $3.43(2.88)$ \\
& 0.40
& $\mathbf{0.00(0.00)}$ & $9.93(1.26)$ & $0.71(0.06)$ 
& $1.75(0.08)$ & $1.67(0.22)$ & $2.69(0.48)$ \\
\midrule
\multirow{7}{*}{Fashion-MNIST}
& 0.10
& $\mathbf{0.00(0.00)}$ & $47.64(2.92)$ & $31.56(1.80)$ 
& $10.73(0.59)$ & $8.20(0.31)$ & $37.66(21.34)$ \\
& 0.15
& $\mathbf{0.00(0.00)}$ & $44.91(5.63)$ & $22.39(2.14)$ 
& $8.20(0.17)$ & $8.18(0.27)$ & $19.94(7.56)$ \\
& 0.20
& $\mathbf{0.00(0.00)}$ & $39.97(3.78)$ & $13.99(0.86)$ 
& $8.54(0.27)$ & $8.72(0.57)$ & $12.25(2.78)$ \\
& 0.25
& $\mathbf{0.00(0.00)}$ & $34.61(4.51)$ & $8.97(0.86)$ 
& $9.96(0.46)$ & $9.74(0.60)$ & $11.84(1.46)$ \\
& 0.30
& $\mathbf{0.00(0.00)}$ & $31.74(3.48)$ & $5.13(0.61)$ 
& $12.59(1.10)$ & $11.26(0.95)$ & $15.48(2.14)$ \\
& 0.35
& $\mathbf{0.00(0.00)}$ & $27.98(3.63)$ & $2.71(0.38)$ 
& $14.79(0.62)$ & $12.37(1.06)$ & $17.68(2.31)$ \\
& 0.40
& $\mathbf{0.00(0.00)}$ & $24.11(2.12)$ & $1.20(0.12)$ 
& $18.31(0.83)$ & $14.91(1.31)$ & $19.89(2.46)$ \\
\midrule
\multirow{7}{*}{KMNIST}
& 0.10
& $\mathbf{0.00(0.00)}$ & $49.39(1.94)$ & $41.64(3.71)$ 
& $16.60(0.56)$ & $8.21(0.35)$ & $18.35(7.46)$ \\
& 0.15
& $\mathbf{0.00(0.00)}$ & $47.25(3.19)$ & $32.37(1.73)$ 
& $11.47(0.50)$ & $7.94(0.25)$ & $11.71(3.46)$ \\
& 0.20
& $\mathbf{0.00(0.00)}$ & $42.36(2.09)$ & $23.70(0.96)$ 
& $9.14(0.23)$ & $7.94(0.19)$ & $12.25(5.62)$ \\
& 0.25
& $\mathbf{0.00(0.00)}$ & $39.94(2.79)$ & $17.43(1.22)$ 
& $8.18(0.27)$ & $7.84(0.38)$ & $12.46(3.66)$ \\
& 0.30
& $\mathbf{0.00(0.00)}$ & $38.23(3.33)$ & $12.85(0.81)$ 
& $7.83(0.15)$ & $8.14(0.36)$ & $11.02(2.26)$ \\
& 0.35
& $\mathbf{0.00(0.00)}$ & $33.38(3.08)$ & $8.90(0.47)$ 
& $8.06(0.30)$ & $8.50(0.36)$ & $11.32(0.82)$ \\
& 0.40
& $\mathbf{0.00(0.00)}$ & $29.03(1.60)$ & $5.69(0.47)$ 
& $8.56(0.31)$ & $8.76(0.26)$ & $11.88(0.91)$ \\
\bottomrule
\end{tabular}
} % \resizebox
\caption{Mean and standard error of rejection ratio of the clean-labeled setting (rescaled to $0-100$).}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table*}[t]
\centering
\resizebox{.95\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
Dataset & $c$ 
& SCE & DEFER & OVA-squared& CS-squared& CS-hinge & CS-sigmoid \\
\midrule
\multirow{7}{*}{Gisette}
& 0.10
& $\mathbf{2.01(0.11)}$ & $3.81(0.15)$ & $2.89(0.39)$ 
& $5.42(0.26)$ & $2.12(0.09)$ & $\mathbf{2.02(0.09)}$ \\
& 0.15
& $\mathbf{2.11(0.15)}$ & $3.70(0.18)$ & $3.35(0.37)$ 
& $6.61(0.24)$ & $\mathbf{2.18(0.14)}$ & $2.24(0.04)$ \\
& 0.20
& $\mathbf{2.12(0.14)}$ & $3.55(0.19)$ & $3.94(0.34)$ 
& $7.35(0.23)$ & $\mathbf{2.13(0.10)}$ & $2.35(0.07)$ \\
& 0.25
& $2.38(0.16)$ & $3.53(0.21)$ & $4.71(0.30)$ 
& $7.81(0.30)$ & $\mathbf{2.17(0.08)}$ & $2.53(0.08)$ \\
& 0.30
& $\mathbf{2.30(0.15)}$ & $3.56(0.16)$ & $5.61(0.33)$ 
& $8.51(0.44)$ & $\mathbf{2.33(0.13)}$ & $2.62(0.10)$ \\
& 0.35
& $\mathbf{2.34(0.13)}$ & $3.44(0.22)$ & $6.98(0.42)$ 
& $8.85(0.39)$ & $\mathbf{2.31(0.15)}$ & $2.83(0.04)$ \\
& 0.40
& $\mathbf{2.47(0.12)}$ & $3.30(0.15)$ & $8.18(0.49)$ 
& $8.87(0.40)$ & $\mathbf{2.42(0.13)}$ & $2.91(0.10)$ \\
\midrule
\multirow{7}{*}{Phishing}
& 0.10
& $2.54(0.51)$ & $0.34(0.04)$ & $0.16(0.00)$ 
& $\mathbf{0.15(0.02)}$ & $1.14(0.11)$ & $2.66(0.20)$ \\
& 0.15
& $2.70(0.57)$ & $0.44(0.02)$ & $\mathbf{0.34(0.01)}$ 
& $2.36(0.04)$ & $2.31(0.12)$ & $2.93(0.14)$ \\
& 0.20
& $2.62(0.37)$ & $\mathbf{0.79(0.05)}$ & $1.00(0.05)$ 
& $3.99(0.02)$ & $3.46(0.11)$ & $3.53(0.15)$ \\
& 0.25
& $3.22(0.46)$ & $\mathbf{0.98(0.05)}$ & $2.01(0.05)$ 
& $5.51(0.04)$ & $3.95(0.07)$ & $4.06(0.16)$ \\
& 0.30
& $3.58(0.81)$ & $\mathbf{1.48(0.02)}$ & $3.30(0.03)$ 
& $6.31(0.03)$ & $4.82(0.20)$ & $4.76(0.15)$ \\
& 0.35
& $3.67(0.53)$ & $\mathbf{1.88(0.05)}$ & $4.35(0.05)$ 
& $6.84(0.02)$ & $5.82(0.15)$ & $5.39(0.14)$ \\
& 0.40
& $3.94(0.43)$ & $\mathbf{2.60(0.04)}$ & $5.97(0.01)$ 
& $7.18(0.04)$ & $6.39(0.05)$ & $6.23(0.17)$ \\
\midrule
\multirow{7}{*}{Spambase}
& 0.10
& $3.71(0.41)$ & $4.65(0.12)$ & $2.33(0.03)$ 
& $\mathbf{1.57(0.14)}$ & $2.48(0.17)$ & $5.31(0.38)$ \\
& 0.15
& $3.70(0.38)$ & $4.84(0.24)$ & $2.36(0.08)$ 
& $\mathbf{1.98(0.21)}$ & $3.45(0.28)$ & $5.94(0.37)$ \\
& 0.20
& $4.19(0.47)$ & $5.31(0.13)$ & $3.69(0.08)$ 
& $\mathbf{3.30(0.12)}$ & $5.04(0.16)$ & $6.50(0.27)$ \\
& 0.25
& $\mathbf{4.39(0.53)}$ & $5.63(0.16)$ & $\mathbf{4.57(0.04)}$ 
& $4.71(0.10)$ & $5.76(0.16)$ & $6.65(0.12)$ \\
& 0.30
& $\mathbf{4.21(0.49)}$ & $6.03(0.14)$ & $5.26(0.07)$ 
& $5.43(0.05)$ & $6.40(0.14)$ & $6.92(0.17)$ \\
& 0.35
& $\mathbf{4.51(0.51)}$ & $6.39(0.07)$ & $5.89(0.06)$ 
& $6.50(0.07)$ & $7.00(0.17)$ & $7.58(0.25)$ \\
& 0.40
& $\mathbf{4.74(0.45)}$ & $6.82(0.13)$ & $7.26(0.05)$ 
& $8.35(0.04)$ & $7.50(0.16)$ & $8.33(0.31)$ \\
\midrule
\multirow{7}{*}{Subj}
& 0.10
& $5.56(0.31)$ & $2.74(0.10)$ & $\mathbf{1.94(0.06)}$ 
& $2.13(0.03)$ & $4.54(0.07)$ & $7.75(0.08)$ \\
& 0.15
& $6.04(0.40)$ & $3.14(0.05)$ & $\mathbf{2.79(0.06)}$ 
& $3.64(0.05)$ & $5.62(0.12)$ & $8.23(0.07)$ \\
& 0.20
& $6.51(0.31)$ & $3.41(0.07)$ & $\mathbf{3.30(0.07)}$ 
& $5.03(0.07)$ & $6.68(0.06)$ & $8.63(0.10)$ \\
& 0.25
& $6.31(0.34)$ & $\mathbf{3.68(0.05)}$ & $\mathbf{3.72(0.04)}$ 
& $6.19(0.07)$ & $7.51(0.07)$ & $9.05(0.11)$ \\
& 0.30
& $6.90(0.50)$ & $\mathbf{4.30(0.10)}$ & $4.81(0.07)$ 
& $7.31(0.07)$ & $8.22(0.08)$ & $9.47(0.10)$ \\
& 0.35
& $6.95(0.50)$ & $\mathbf{4.98(0.07)}$ & $6.04(0.06)$ 
& $8.42(0.08)$ & $8.99(0.07)$ & $9.76(0.06)$ \\
& 0.40
& $7.16(0.32)$ & $\mathbf{5.59(0.08)}$ & $7.67(0.07)$ 
& $9.37(0.12)$ & $9.72(0.10)$ & $10.25(0.08)$ \\
\midrule
\multirow{7}{*}{Twonorm}
& 0.10
& $0.54(0.11)$ & $\mathbf{0.00(0.00)}$ & $\mathbf{0.00(0.00)}$ 
& $0.08(0.02)$ & $0.84(0.12)$ & $1.09(0.10)$ \\
& 0.15
& $0.66(0.20)$ & $\mathbf{0.00(0.00)}$ & $\mathbf{0.00(0.00)}$ 
& $0.42(0.01)$ & $0.93(0.07)$ & $1.02(0.14)$ \\
& 0.20
& $0.66(0.15)$ & $\mathbf{0.00(0.00)}$ & $0.04(0.00)$ 
& $0.76(0.01)$ & $1.08(0.11)$ & $1.06(0.12)$ \\
& 0.25
& $0.75(0.12)$ & $\mathbf{0.00(0.00)}$ & $0.07(0.00)$ 
& $0.95(0.02)$ & $1.23(0.08)$ & $1.15(0.10)$ \\
& 0.30
& $0.73(0.12)$ & $\mathbf{0.04(0.00)}$ & $0.13(0.00)$ 
& $1.19(0.01)$ & $1.33(0.04)$ & $1.22(0.06)$ \\
& 0.35
& $0.85(0.20)$ & $\mathbf{0.04(0.00)}$ & $0.30(0.00)$ 
& $1.45(0.02)$ & $1.54(0.07)$ & $1.41(0.09)$ \\
& 0.40
& $0.89(0.15)$ & $\mathbf{0.07(0.01)}$ & $0.69(0.01)$ 
& $1.69(0.02)$ & $1.73(0.08)$ & $1.65(0.10)$ \\
\midrule
\multirow{7}{*}{MNIST}
& 0.10
& $0.85(0.08)$ & $0.03(0.02)$ & $\mathbf{0.01(0.01)}$ 
& $0.39(0.03)$ & $0.28(0.04)$ & $0.50(0.20)$ \\
& 0.15
& $0.82(0.09)$ & $\mathbf{0.02(0.01)}$ & $0.04(0.02)$ 
& $0.44(0.03)$ & $0.30(0.03)$ & $0.50(0.11)$ \\
& 0.20
& $0.83(0.07)$ & $\mathbf{0.03(0.01)}$ & $0.09(0.02)$ 
& $0.42(0.03)$ & $0.29(0.04)$ & $0.42(0.08)$ \\
& 0.25
& $0.88(0.12)$ & $\mathbf{0.04(0.02)}$ & $0.16(0.03)$ 
& $0.42(0.03)$ & $0.29(0.03)$ & $0.41(0.06)$ \\
& 0.30
& $0.84(0.07)$ & $\mathbf{0.04(0.01)}$ & $0.25(0.05)$ 
& $0.43(0.04)$ & $0.30(0.04)$ & $0.47(0.10)$ \\
& 0.35
& $0.86(0.08)$ & $\mathbf{0.05(0.01)}$ & $0.42(0.02)$ 
& $0.41(0.05)$ & $0.29(0.02)$ & $0.42(0.09)$ \\
& 0.40
& $0.83(0.09)$ & $\mathbf{0.06(0.02)}$ & $0.51(0.04)$ 
& $0.37(0.06)$ & $0.31(0.05)$ & $0.41(0.07)$ \\
\midrule
\multirow{7}{*}{Fashion-MNIST}
& 0.10
& $8.49(0.16)$ & $\mathbf{1.90(0.35)}$ & $\mathbf{2.13(0.24)}$ 
& $4.27(0.16)$ & $4.58(0.18)$ & $4.11(1.64)$ \\
& 0.15
& $8.37(0.17)$ & $\mathbf{2.04(0.24)}$ & $2.87(0.30)$ 
& $4.81(0.14)$ & $4.74(0.12)$ & $5.75(0.71)$ \\
& 0.20
& $8.37(0.18)$ & $\mathbf{2.09(0.31)}$ & $4.03(0.23)$ 
& $4.83(0.11)$ & $4.72(0.10)$ & $5.46(0.44)$ \\
& 0.25
& $8.51(0.24)$ & $\mathbf{2.34(0.38)}$ & $4.94(0.15)$ 
& $4.58(0.07)$ & $4.57(0.14)$ & $5.16(0.88)$ \\
& 0.30
& $8.46(0.14)$ & $\mathbf{2.49(0.31)}$ & $6.00(0.23)$ 
& $4.14(0.27)$ & $4.45(0.20)$ & $4.26(0.38)$ \\
& 0.35
& $8.51(0.15)$ & $\mathbf{2.66(0.28)}$ & $6.75(0.16)$ 
& $3.71(0.14)$ & $4.19(0.16)$ & $4.19(1.19)$ \\
& 0.40
& $8.43(0.15)$ & $\mathbf{3.02(0.23)}$ & $7.48(0.18)$ 
& $\mathbf{3.14(0.21)}$ & $3.71(0.22)$ & $3.41(0.55)$ \\
\midrule
\multirow{7}{*}{KMNIST}
& 0.10
& $5.81(0.23)$ & $\mathbf{0.40(0.08)}$ & $\mathbf{0.34(0.06)}$ 
& $1.54(0.10)$ & $2.04(0.13)$ & $2.48(0.33)$ \\
& 0.15
& $5.71(0.23)$ & $\mathbf{0.44(0.05)}$ & $\mathbf{0.48(0.09)}$ 
& $2.03(0.11)$ & $2.25(0.15)$ & $2.85(0.16)$ \\
& 0.20
& $5.70(0.24)$ & $\mathbf{0.48(0.13)}$ & $0.81(0.09)$ 
& $2.43(0.11)$ & $2.30(0.13)$ & $3.20(0.41)$ \\
& 0.25
& $5.82(0.16)$ & $\mathbf{0.55(0.08)}$ & $1.18(0.15)$ 
& $2.61(0.12)$ & $2.44(0.13)$ & $3.39(0.38)$ \\
& 0.30
& $5.79(0.22)$ & $\mathbf{0.50(0.08)}$ & $1.79(0.13)$ 
& $2.79(0.12)$ & $2.50(0.17)$ & $3.12(0.24)$ \\
& 0.35
& $5.79(0.24)$ & $\mathbf{0.61(0.11)}$ & $2.35(0.17)$ 
& $2.99(0.15)$ & $2.58(0.14)$ & $3.25(0.24)$ \\
& 0.40
& $5.69(0.21)$ & $\mathbf{0.76(0.12)}$ & $3.33(0.15)$ 
& $2.94(0.14)$ & $2.63(0.17)$ & $3.37(0.23)$ \\
\bottomrule
\end{tabular}
} % \resizebox
\caption{Mean and standard error of $0\text{-}1$ risk for accepted data of the clean-labeled setting (rescaled to $0-100$).}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table*}[t]
\centering
\resizebox{.95\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
Dataset & $c$ 
& SCE & DEFER & OVA-squared& CS-squared& CS-hinge & CS-sigmoid \\
\midrule
\multirow{7}{*}{Gisette}
& 0.10
& $22.46(1.46)$ & $22.10(1.23)$ & $25.80(0.77)$ 
& $30.20(1.16)$ & $24.88(0.83)$ & $\mathbf{8.22(0.50)}$ \\
& 0.15
& $23.48(1.02)$ & $23.33(0.76)$ & $29.20(1.29)$ 
& $33.17(1.09)$ & $26.69(0.93)$ & $\mathbf{9.70(0.87)}$ \\
& 0.20
& $24.93(1.17)$ & $24.98(1.13)$ & $31.93(0.55)$ 
& $34.51(0.94)$ & $28.27(0.96)$ & $\mathbf{10.74(0.88)}$ \\
& 0.25
& $26.04(1.28)$ & $27.30(0.63)$ & $34.05(0.53)$ 
& $36.19(1.22)$ & $28.47(0.94)$ & $\mathbf{12.51(0.67)}$ \\
& 0.30
& $26.88(1.18)$ & $28.74(1.02)$ & $36.03(0.96)$ 
& $36.68(0.98)$ & $29.74(1.26)$ & $\mathbf{14.08(0.46)}$ \\
& 0.35
& $27.40(1.41)$ & $30.18(0.84)$ & $37.69(1.02)$ 
& $37.97(1.18)$ & $29.17(0.87)$ & $\mathbf{14.93(1.05)}$ \\
& 0.40
& $28.18(0.66)$ & $31.88(0.81)$ & $38.26(0.68)$ 
& $38.81(1.14)$ & $30.57(1.00)$ & $\mathbf{16.61(1.28)}$ \\
\midrule
\multirow{7}{*}{Phishing}
& 0.10
& $\mathbf{8.90(0.20)}$ & $9.09(0.19)$ & $9.91(0.05)$ 
& $10.00(0.00)$ & $10.00(0.00)$ & $\mathbf{9.26(3.06)}$ \\
& 0.15
& $12.98(0.51)$ & $12.74(0.32)$ & $14.18(0.15)$ 
& $14.99(0.01)$ & $15.00(0.00)$ & $\mathbf{10.12(3.02)}$ \\
& 0.20
& $16.27(0.84)$ & $15.25(0.36)$ & $16.89(0.49)$ 
& $19.17(0.29)$ & $19.74(0.79)$ & $\mathbf{9.54(1.88)}$ \\
& 0.25
& $19.82(1.16)$ & $16.80(0.30)$ & $18.32(0.42)$ 
& $19.54(0.70)$ & $22.69(1.51)$ & $\mathbf{9.60(2.35)}$ \\
& 0.30
& $23.02(1.37)$ & $17.07(0.28)$ & $17.29(0.71)$ 
& $16.16(0.67)$ & $19.12(1.45)$ & $\mathbf{8.96(0.34)}$ \\
& 0.35
& $26.33(2.27)$ & $15.28(0.44)$ & $14.29(0.46)$ 
& $12.60(0.59)$ & $10.22(0.47)$ & $\mathbf{9.04(0.27)}$ \\
& 0.40
& $28.49(2.24)$ & $12.93(0.21)$ & $11.02(0.28)$ 
& $9.89(0.26)$ & $10.10(0.24)$ & $\mathbf{8.90(0.34)}$ \\
\midrule
\multirow{7}{*}{Spambase}
& 0.10
& $9.52(0.19)$ & $9.83(0.16)$ & $9.71(0.11)$ 
& $9.56(0.20)$ & $8.32(0.19)$ & $\mathbf{7.39(0.31)}$ \\
& 0.15
& $13.95(0.35)$ & $14.21(0.25)$ & $14.22(0.16)$ 
& $13.82(0.23)$ & $12.46(0.37)$ & $\mathbf{9.52(0.29)}$ \\
& 0.20
& $17.58(0.45)$ & $17.83(0.41)$ & $18.10(0.37)$ 
& $18.02(0.66)$ & $15.43(0.97)$ & $\mathbf{11.41(0.24)}$ \\
& 0.25
& $21.41(0.90)$ & $20.45(0.62)$ & $21.28(0.73)$ 
& $19.98(0.67)$ & $18.64(0.56)$ & $\mathbf{12.45(0.52)}$ \\
& 0.30
& $25.07(1.25)$ & $20.10(0.76)$ & $21.77(0.70)$ 
& $21.54(0.67)$ & $20.22(1.27)$ & $\mathbf{12.71(0.86)}$ \\
& 0.35
& $29.14(1.21)$ & $19.70(0.95)$ & $20.21(1.15)$ 
& $19.17(0.93)$ & $18.92(1.55)$ & $\mathbf{11.76(0.45)}$ \\
& 0.40
& $31.02(1.51)$ & $17.32(0.72)$ & $16.57(1.21)$ 
& $16.09(1.11)$ & $14.23(1.25)$ & $\mathbf{10.35(0.29)}$ \\
\midrule
\multirow{7}{*}{Subj}
& 0.10
& $9.42(0.18)$ & $9.08(0.10)$ & $9.65(0.07)$ 
& $10.00(0.00)$ & $10.00(0.00)$ & $\mathbf{7.58(0.25)}$ \\
& 0.15
& $13.65(0.29)$ & $13.08(0.22)$ & $13.92(0.16)$ 
& $14.93(0.02)$ & $15.00(0.00)$ & $\mathbf{9.15(0.16)}$ \\
& 0.20
& $17.20(0.45)$ & $16.47(0.18)$ & $17.56(0.32)$ 
& $18.78(0.28)$ & $20.00(0.00)$ & $\mathbf{10.38(0.34)}$ \\
& 0.25
& $21.29(0.60)$ & $18.79(0.58)$ & $19.64(0.26)$ 
& $20.76(0.51)$ & $25.00(0.00)$ & $\mathbf{11.09(0.21)}$ \\
& 0.30
& $24.46(0.49)$ & $19.95(0.27)$ & $20.10(0.56)$ 
& $19.84(0.37)$ & $25.20(2.53)$ & $\mathbf{11.63(0.19)}$ \\
& 0.35
& $27.45(1.22)$ & $20.07(0.47)$ & $18.77(0.38)$ 
& $18.16(0.84)$ & $17.36(0.70)$ & $\mathbf{12.14(0.26)}$ \\
& 0.40
& $30.33(1.26)$ & $18.62(0.41)$ & $17.22(0.39)$ 
& $16.53(0.53)$ & $14.68(0.35)$ & $\mathbf{12.44(0.28)}$ \\
\midrule
\multirow{7}{*}{Twonorm}
& 0.10
& $8.25(0.35)$ & $8.74(0.18)$ & $9.71(0.11)$ 
& $10.00(0.00)$ & $10.00(0.00)$ & $\mathbf{1.50(0.15)}$ \\
& 0.15
& $11.98(0.75)$ & $12.30(0.33)$ & $13.80(0.18)$ 
& $14.97(0.01)$ & $15.00(0.00)$ & $\mathbf{1.65(0.10)}$ \\
& 0.20
& $15.12(0.70)$ & $14.74(0.39)$ & $16.61(0.53)$ 
& $18.43(0.31)$ & $20.00(0.00)$ & $\mathbf{1.88(0.08)}$ \\
& 0.25
& $18.79(1.58)$ & $16.08(0.34)$ & $17.48(1.07)$ 
& $18.23(1.03)$ & $23.17(1.81)$ & $\mathbf{2.14(0.08)}$ \\
& 0.30
& $21.93(0.88)$ & $16.03(0.40)$ & $15.12(0.78)$ 
& $13.31(1.04)$ & $8.23(2.19)$ & $\mathbf{2.23(0.09)}$ \\
& 0.35
& $23.26(2.68)$ & $14.28(0.65)$ & $11.56(0.34)$ 
& $9.23(0.72)$ & $4.36(0.16)$ & $\mathbf{2.33(0.09)}$ \\
& 0.40
& $25.32(3.90)$ & $11.06(0.34)$ & $7.11(0.38)$ 
& $5.47(0.38)$ & $3.08(0.13)$ & $\mathbf{2.42(0.06)}$ \\
\midrule
\multirow{7}{*}{MNIST}
& 0.10
& $2.38(0.10)$ & $7.86(0.39)$ & $3.71(0.52)$ 
& $1.18(0.11)$ & $\mathbf{0.57(0.04)}$ & $7.31(2.16)$ \\
& 0.15
& $2.23(0.20)$ & $10.74(0.92)$ & $3.11(0.43)$ 
& $0.94(0.06)$ & $\mathbf{0.65(0.03)}$ & $3.00(1.51)$ \\
& 0.20
& $2.37(0.09)$ & $12.67(0.99)$ & $2.43(0.22)$ 
& $1.02(0.08)$ & $\mathbf{0.71(0.04)}$ & $2.10(1.31)$ \\
& 0.25
& $2.33(0.18)$ & $14.90(1.15)$ & $1.93(0.19)$ 
& $1.10(0.07)$ & $\mathbf{0.81(0.04)}$ & $1.77(1.14)$ \\
& 0.30
& $2.41(0.17)$ & $14.79(1.99)$ & $1.76(0.11)$ 
& $1.25(0.06)$ & $\mathbf{0.92(0.05)}$ & $1.52(0.94)$ \\
& 0.35
& $2.30(0.13)$ & $14.72(2.51)$ & $1.54(0.09)$ 
& $1.63(0.08)$ & $\mathbf{1.13(0.07)}$ & $1.83(0.96)$ \\
& 0.40
& $2.39(0.22)$ & $13.57(1.58)$ & $\mathbf{1.51(0.14)}$ 
& $2.53(0.13)$ & $\mathbf{1.47(0.05)}$ & $1.99(0.50)$ \\
\midrule
\multirow{7}{*}{Fashion-MNIST}
& 0.10
& $11.46(0.21)$ & $8.11(0.27)$ & $6.14(0.29)$ 
& $4.23(0.09)$ & $\mathbf{4.15(0.07)}$ & $9.08(1.23)$ \\
& 0.15
& $11.49(0.40)$ & $11.51(0.59)$ & $7.37(0.31)$ 
& $\mathbf{5.63(0.11)}$ & $\mathbf{5.61(0.13)}$ & $8.19(0.98)$ \\
& 0.20
& $11.78(0.30)$ & $13.82(0.48)$ & $8.43(0.22)$ 
& $6.66(0.16)$ & $\mathbf{6.46(0.11)}$ & $9.46(1.38)$ \\
& 0.25
& $11.57(0.46)$ & $16.52(0.95)$ & $8.88(0.22)$ 
& $7.55(0.14)$ & $\mathbf{7.08(0.18)}$ & $8.93(1.47)$ \\
& 0.30
& $11.68(0.37)$ & $18.47(1.17)$ & $9.35(0.21)$ 
& $8.57(0.15)$ & $\mathbf{7.92(0.18)}$ & $8.68(0.81)$ \\
& 0.35
& $11.61(0.31)$ & $19.92(1.38)$ & $9.70(0.18)$ 
& $10.01(0.19)$ & $\mathbf{9.17(0.19)}$ & $9.79(0.26)$ \\
& 0.40
& $11.64(0.31)$ & $20.20(1.44)$ & $\mathbf{10.01(0.23)}$ 
& $12.12(0.31)$ & $10.87(0.28)$ & $11.50(0.65)$ \\
\midrule
\multirow{7}{*}{KMNIST}
& 0.10
& $11.26(0.34)$ & $7.77(0.19)$ & $6.22(0.40)$ 
& $4.17(0.17)$ & $\mathbf{2.99(0.08)}$ & $9.09(0.95)$ \\
& 0.15
& $11.12(0.26)$ & $11.21(0.41)$ & $7.32(0.26)$ 
& $4.62(0.15)$ & $\mathbf{3.67(0.11)}$ & $5.96(1.24)$ \\
& 0.20
& $11.53(0.46)$ & $14.07(0.62)$ & $7.78(0.29)$ 
& $5.30(0.15)$ & $\mathbf{4.39(0.14)}$ & $6.63(0.71)$ \\
& 0.25
& $11.43(0.46)$ & $16.23(0.87)$ & $8.30(0.35)$ 
& $6.02(0.21)$ & $\mathbf{4.97(0.16)}$ & $7.17(1.42)$ \\
& 0.30
& $11.37(0.28)$ & $18.75(0.83)$ & $8.41(0.25)$ 
& $7.21(0.24)$ & $\mathbf{5.75(0.21)}$ & $6.72(0.72)$ \\
& 0.35
& $11.36(0.29)$ & $20.65(0.70)$ & $8.93(0.25)$ 
& $8.83(0.19)$ & $\mathbf{6.73(0.14)}$ & $7.79(0.43)$ \\
& 0.40
& $11.59(0.45)$ & $20.78(0.73)$ & $9.15(0.29)$ 
& $11.30(0.43)$ & $\mathbf{8.22(0.16)}$ & $8.90(0.59)$ \\
\bottomrule
\end{tabular}
} % \resizebox
\caption{Mean and standard error of $0\text{-}1\text{-}c$ risk of the noisy-labeled setting (rescaled to $0-100$).}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table*}[t]
\centering
\resizebox{.95\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
Dataset & $c$ 
& SCE & DEFER & OVA-squared& CS-squared& CS-hinge & CS-sigmoid \\
\midrule
\multirow{7}{*}{Gisette}
& 0.10
& $18.30(0.94)$ & $35.81(1.01)$ & $36.73(1.04)$ 
& $17.78(0.75)$ & $\mathbf{13.37(0.55)}$ & $22.16(0.97)$ \\
& 0.15
& $16.94(0.48)$ & $35.64(1.23)$ & $32.49(0.73)$ 
& $14.69(0.50)$ & $\mathbf{10.48(0.81)}$ & $20.14(0.72)$ \\
& 0.20
& $16.38(0.44)$ & $36.39(0.56)$ & $28.67(0.46)$ 
& $11.78(0.71)$ & $\mathbf{9.38(0.62)}$ & $17.97(1.06)$ \\
& 0.25
& $15.60(0.62)$ & $36.18(1.04)$ & $23.38(0.79)$ 
& $10.09(0.60)$ & $\mathbf{8.49(0.58)}$ & $16.43(1.02)$ \\
& 0.30
& $14.47(0.75)$ & $36.14(1.18)$ & $19.27(0.63)$ 
& $8.42(0.59)$ & $\mathbf{7.75(0.39)}$ & $15.55(0.73)$ \\
& 0.35
& $13.41(0.62)$ & $35.95(1.48)$ & $14.51(0.67)$ 
& $7.67(0.58)$ & $\mathbf{7.24(0.31)}$ & $14.04(1.53)$ \\
& 0.40
& $12.28(0.72)$ & $36.62(0.88)$ & $9.80(0.38)$ 
& $\mathbf{6.67(0.65)}$ & $\mathbf{6.63(0.40)}$ & $12.16(0.91)$ \\
\midrule
\multirow{7}{*}{Phishing}
& 0.10
& $86.94(2.80)$ & $90.87(1.85)$ & $99.08(0.55)$ 
& $100.00(0.00)$ & $100.00(0.00)$ & $\mathbf{70.25(7.45)}$ \\
& 0.15
& $85.18(3.66)$ & $84.84(2.06)$ & $94.55(1.01)$ 
& $99.94(0.06)$ & $100.00(0.00)$ & $\mathbf{57.85(6.92)}$ \\
& 0.20
& $79.29(4.80)$ & $76.16(1.78)$ & $84.46(2.48)$ 
& $95.85(1.47)$ & $98.68(3.96)$ & $\mathbf{43.66(6.22)}$ \\
& 0.25
& $77.56(4.92)$ & $67.00(1.24)$ & $73.24(1.68)$ 
& $78.14(2.79)$ & $90.77(6.04)$ & $\mathbf{31.58(6.14)}$ \\
& 0.30
& $74.95(5.02)$ & $56.31(1.00)$ & $57.14(2.52)$ 
& $53.17(2.42)$ & $63.33(5.40)$ & $\mathbf{22.23(1.58)}$ \\
& 0.35
& $73.58(7.10)$ & $41.94(1.41)$ & $38.62(1.48)$ 
& $32.31(2.66)$ & $\mathbf{15.87(2.26)}$ & $\mathbf{16.53(0.92)}$ \\
& 0.40
& $69.29(6.31)$ & $27.69(1.12)$ & $20.99(0.88)$ 
& $15.99(1.66)$ & $\mathbf{6.05(0.57)}$ & $11.88(1.10)$ \\
\midrule
\multirow{7}{*}{Spambase}
& 0.10
& $88.23(2.01)$ & $93.95(1.12)$ & $95.85(0.77)$ 
& $93.04(1.77)$ & $77.77(2.66)$ & $\mathbf{48.58(2.04)}$ \\
& 0.15
& $87.70(2.71)$ & $91.11(1.17)$ & $93.49(1.32)$ 
& $89.49(1.79)$ & $80.11(1.86)$ & $\mathbf{44.03(2.39)}$ \\
& 0.20
& $83.76(2.81)$ & $85.19(1.85)$ & $88.74(2.03)$ 
& $87.94(3.18)$ & $74.39(5.73)$ & $\mathbf{41.06(2.23)}$ \\
& 0.25
& $81.28(3.89)$ & $77.53(2.73)$ & $82.39(2.88)$ 
& $76.87(2.80)$ & $72.49(2.22)$ & $\mathbf{35.35(1.56)}$ \\
& 0.30
& $79.90(4.22)$ & $60.89(3.90)$ & $69.07(2.53)$ 
& $68.47(2.25)$ & $64.64(5.04)$ & $\mathbf{28.90(3.74)}$ \\
& 0.35
& $79.86(4.22)$ & $48.24(4.13)$ & $51.50(3.79)$ 
& $47.50(3.48)$ & $48.65(5.41)$ & $\mathbf{18.74(1.54)}$ \\
& 0.40
& $73.80(3.73)$ & $31.76(2.16)$ & $29.69(3.31)$ 
& $29.09(3.66)$ & $22.67(5.29)$ & $\mathbf{9.29(0.57)}$ \\
\midrule
\multirow{7}{*}{Subj}
& 0.10
& $84.30(2.50)$ & $88.98(1.04)$ & $96.20(0.73)$ 
& $100.00(0.01)$ & $100.00(0.00)$ & $\mathbf{38.52(6.17)}$ \\
& 0.15
& $84.50(3.28)$ & $84.93(1.80)$ & $92.26(1.17)$ 
& $99.54(0.11)$ & $100.00(0.00)$ & $\mathbf{31.15(2.30)}$ \\
& 0.20
& $78.97(2.28)$ & $79.53(1.07)$ & $86.83(1.74)$ 
& $93.60(1.43)$ & $100.00(0.00)$ & $\mathbf{25.22(1.72)}$ \\
& 0.25
& $78.48(3.46)$ & $71.40(2.17)$ & $76.49(1.23)$ 
& $81.75(2.21)$ & $100.00(0.00)$ & $\mathbf{19.91(2.13)}$ \\
& 0.30
& $76.75(2.74)$ & $62.04(1.17)$ & $63.28(2.17)$ 
& $62.07(1.67)$ & $82.49(9.55)$ & $\mathbf{14.98(1.33)}$ \\
& 0.35
& $72.47(4.77)$ & $51.06(1.37)$ & $46.99(1.53)$ 
& $44.52(2.84)$ & $40.96(2.64)$ & $\mathbf{12.00(1.08)}$ \\
& 0.40
& $70.90(3.80)$ & $37.85(1.10)$ & $31.59(1.23)$ 
& $28.53(1.37)$ & $22.49(1.24)$ & $\mathbf{8.90(0.60)}$ \\
\midrule
\multirow{7}{*}{Twonorm}
& 0.10
& $82.22(3.62)$ & $87.38(1.76)$ & $97.05(1.06)$ 
& $100.00(0.00)$ & $100.00(0.00)$ & $\mathbf{10.35(2.45)}$ \\
& 0.15
& $79.35(5.14)$ & $81.98(2.19)$ & $92.00(1.17)$ 
& $99.80(0.09)$ & $100.00(0.00)$ & $\mathbf{5.96(1.10)}$ \\
& 0.20
& $75.07(3.66)$ & $73.68(1.93)$ & $83.07(2.63)$ 
& $92.15(1.54)$ & $100.00(0.00)$ & $\mathbf{5.51(0.96)}$ \\
& 0.25
& $74.67(6.60)$ & $64.32(1.37)$ & $69.93(4.27)$ 
& $72.91(4.11)$ & $92.66(7.24)$ & $\mathbf{4.67(0.65)}$ \\
& 0.30
& $72.70(3.04)$ & $53.39(1.33)$ & $50.40(2.64)$ 
& $44.32(3.49)$ & $27.21(7.42)$ & $\mathbf{4.16(0.61)}$ \\
& 0.35
& $65.96(7.76)$ & $40.73(1.86)$ & $32.95(0.96)$ 
& $26.13(2.06)$ & $11.48(0.52)$ & $\mathbf{3.48(0.45)}$ \\
& 0.40
& $62.56(10.18)$ & $27.49(0.87)$ & $17.25(0.91)$ 
& $12.93(1.00)$ & $5.98(0.32)$ & $\mathbf{3.04(0.34)}$ \\
\midrule
\multirow{7}{*}{MNIST}
& 0.10
& $\mathbf{0.06(0.02)}$ & $78.52(3.87)$ & $36.82(5.27)$ 
& $11.09(1.23)$ & $3.92(0.42)$ & $70.58(23.41)$ \\
& 0.15
& $\mathbf{0.02(0.02)}$ & $71.59(6.12)$ & $20.28(2.96)$ 
& $4.46(0.45)$ & $2.24(0.12)$ & $16.82(10.38)$ \\
& 0.20
& $\mathbf{0.02(0.01)}$ & $63.26(4.97)$ & $11.35(1.12)$ 
& $2.97(0.44)$ & $1.56(0.11)$ & $7.98(6.28)$ \\
& 0.25
& $\mathbf{0.02(0.02)}$ & $59.53(4.61)$ & $6.43(0.81)$ 
& $2.27(0.25)$ & $1.44(0.08)$ & $5.18(4.38)$ \\
& 0.30
& $\mathbf{0.01(0.01)}$ & $49.20(6.66)$ & $4.10(0.39)$ 
& $2.22(0.15)$ & $1.49(0.10)$ & $3.39(2.92)$ \\
& 0.35
& $\mathbf{0.00(0.01)}$ & $41.89(7.18)$ & $1.96(0.25)$ 
& $2.97(0.21)$ & $1.89(0.12)$ & $3.81(2.53)$ \\
& 0.40
& $\mathbf{0.00(0.00)}$ & $33.77(3.96)$ & $0.87(0.18)$ 
& $5.07(0.28)$ & $2.55(0.17)$ & $3.72(1.17)$ \\
\midrule
\multirow{7}{*}{Fashion-MNIST}
& 0.10
& $\mathbf{0.20(0.14)}$ & $76.85(2.42)$ & $46.57(3.49)$ 
& $28.29(0.87)$ & $18.98(1.05)$ & $87.66(15.86)$ \\
& 0.15
& $\mathbf{0.10(0.06)}$ & $73.39(4.06)$ & $32.95(2.97)$ 
& $14.97(0.88)$ & $11.44(0.46)$ & $34.15(8.86)$ \\
& 0.20
& $\mathbf{0.06(0.02)}$ & $65.29(3.17)$ & $23.56(2.02)$ 
& $10.66(0.59)$ & $9.07(0.26)$ & $24.48(8.32)$ \\
& 0.25
& $\mathbf{0.05(0.04)}$ & $63.05(3.84)$ & $13.30(1.18)$ 
& $10.58(0.36)$ & $9.55(0.65)$ & $13.40(4.64)$ \\
& 0.30
& $\mathbf{0.03(0.03)}$ & $58.12(4.56)$ & $8.07(1.21)$ 
& $13.12(1.02)$ & $11.98(0.88)$ & $12.99(2.96)$ \\
& 0.35
& $\mathbf{0.02(0.01)}$ & $53.05(4.70)$ & $4.55(0.73)$ 
& $17.19(1.52)$ & $15.28(0.93)$ & $17.58(1.44)$ \\
& 0.40
& $\mathbf{0.01(0.01)}$ & $46.54(4.07)$ & $1.68(0.30)$ 
& $22.60(1.30)$ & $19.39(1.31)$ & $21.18(2.42)$ \\
\midrule
\multirow{7}{*}{KMNIST}
& 0.10
& $\mathbf{0.36(0.09)}$ & $76.70(2.08)$ & $59.31(4.56)$ 
& $38.07(2.20)$ & $23.09(1.01)$ & $85.30(15.16)$ \\
& 0.15
& $\mathbf{0.21(0.07)}$ & $73.89(2.91)$ & $44.46(2.27)$ 
& $23.55(1.57)$ & $15.10(0.74)$ & $23.70(8.11)$ \\
& 0.20
& $\mathbf{0.20(0.08)}$ & $69.46(3.23)$ & $33.08(2.28)$ 
& $16.31(0.76)$ & $11.25(0.45)$ & $19.17(4.47)$ \\
& 0.25
& $\mathbf{0.11(0.05)}$ & $63.92(3.71)$ & $24.75(1.64)$ 
& $12.96(0.53)$ & $9.58(0.30)$ & $15.72(5.20)$ \\
& 0.30
& $\mathbf{0.09(0.04)}$ & $61.55(2.88)$ & $17.33(1.17)$ 
& $12.15(0.45)$ & $9.23(0.16)$ & $12.31(2.63)$ \\
& 0.35
& $\mathbf{0.05(0.03)}$ & $57.98(2.09)$ & $10.50(1.09)$ 
& $13.84(0.47)$ & $10.09(0.29)$ & $12.87(0.90)$ \\
& 0.40
& $\mathbf{0.02(0.01)}$ & $50.57(1.81)$ & $5.81(0.70)$ 
& $18.94(1.01)$ & $13.01(0.62)$ & $13.93(1.47)$ \\
\bottomrule
\end{tabular}
} % \resizebox
\caption{Mean and standard error of rejection ratio of the noisy-labeled setting (rescaled to $0-100$).}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table*}[t]
\centering
\resizebox{.95\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
Dataset & $c$ 
& SCE & DEFER & OVA-squared& CS-squared& CS-hinge & CS-sigmoid \\
\midrule
\multirow{7}{*}{Gisette}
& 0.10
& $25.26(1.80)$ & $28.86(1.96)$ & $34.99(1.40)$ 
& $34.57(1.42)$ & $27.18(0.94)$ & $\mathbf{7.73(0.61)}$ \\
& 0.15
& $25.21(1.20)$ & $27.94(1.20)$ & $36.04(2.00)$ 
& $36.29(1.20)$ & $28.06(1.03)$ & $\mathbf{8.36(1.06)}$ \\
& 0.20
& $25.90(1.41)$ & $27.83(1.81)$ & $36.72(0.77)$ 
& $36.44(1.07)$ & $29.12(1.05)$ & $\mathbf{8.71(1.03)}$ \\
& 0.25
& $26.25(1.52)$ & $28.62(1.01)$ & $36.82(0.72)$ 
& $37.45(1.38)$ & $28.80(1.03)$ & $\mathbf{10.05(0.85)}$ \\
& 0.30
& $26.36(1.35)$ & $28.03(1.60)$ & $37.46(1.18)$ 
& $37.29(1.09)$ & $29.72(1.37)$ & $\mathbf{11.15(0.43)}$ \\
& 0.35
& $26.22(1.60)$ & $27.49(1.20)$ & $38.14(1.18)$ 
& $38.22(1.26)$ & $28.72(0.94)$ & $\mathbf{11.66(0.99)}$ \\
& 0.40
& $26.53(0.71)$ & $27.18(1.24)$ & $38.07(0.76)$ 
& $38.72(1.22)$ & $29.90(1.08)$ & $\mathbf{13.38(1.27)}$ \\
\midrule
\multirow{7}{*}{Phishing}
& 0.10
& $1.40(1.23)$ & $\mathbf{0.00(0.00)}$ & $\mathbf{0.00(0.00)}$ 
& $\mathbf{0.00(0.00)}$ & $\mathbf{0.00(0.00)}$ & $8.77(10.59)$ \\
& 0.15
& $1.35(0.81)$ & $0.09(0.16)$ & $\mathbf{0.00(0.00)}$ 
& $\mathbf{0.00(0.00)}$ & $\mathbf{0.00(0.00)}$ & $4.23(7.06)$ \\
& 0.20
& $1.97(0.72)$ & $0.09(0.10)$ & $\mathbf{0.01(0.03)}$ 
& $\mathbf{0.00(0.00)}$ & $\mathbf{0.00(0.00)}$ & $1.60(2.04)$ \\
& 0.25
& $1.91(0.69)$ & $0.14(0.07)$ & $0.04(0.06)$ 
& $\mathbf{0.03(0.08)}$ & $\mathbf{0.00(0.00)}$ & $2.65(1.87)$ \\
& 0.30
& $2.09(1.00)$ & $\mathbf{0.40(0.11)}$ & $\mathbf{0.33(0.20)}$ 
& $\mathbf{0.45(0.18)}$ & $\mathbf{0.27(0.60)}$ & $2.94(0.40)$ \\
& 0.35
& $2.14(0.94)$ & $\mathbf{1.02(0.14)}$ & $1.25(0.22)$ 
& $1.88(0.67)$ & $5.54(0.36)$ & $3.90(0.31)$ \\
& 0.40
& $\mathbf{2.41(0.89)}$ & $\mathbf{2.56(0.34)}$ & $3.32(0.32)$ 
& $4.15(0.46)$ & $8.17(0.44)$ & $4.71(0.25)$ \\
\midrule
\multirow{7}{*}{Spambase}
& 0.10
& $6.01(1.47)$ & $7.44(2.54)$ & $\mathbf{3.06(1.41)}$ 
& $\mathbf{3.80(2.46)}$ & $\mathbf{2.40(0.80)}$ & $4.92(0.65)$ \\
& 0.15
& $6.54(2.18)$ & $6.16(2.52)$ & $\mathbf{3.03(1.40)}$ 
& $3.75(1.13)$ & $\mathbf{2.25(0.96)}$ & $5.20(0.60)$ \\
& 0.20
& $5.06(1.61)$ & $5.39(1.63)$ & $3.15(0.95)$ 
& $3.79(1.67)$ & $\mathbf{2.11(0.45)}$ & $5.41(0.61)$ \\
& 0.25
& $5.96(1.88)$ & $4.78(0.88)$ & $3.98(1.15)$ 
& $3.31(0.81)$ & $\mathbf{1.91(0.54)}$ & $5.60(0.56)$ \\
& 0.30
& $5.69(1.91)$ & $4.64(0.73)$ & $3.40(0.85)$ 
& $3.18(0.56)$ & $\mathbf{2.28(0.65)}$ & $5.67(0.47)$ \\
& 0.35
& $5.84(2.01)$ & $5.39(1.01)$ & $4.49(0.79)$ 
& $4.83(0.88)$ & $\mathbf{3.65(0.80)}$ & $6.39(0.53)$ \\
& 0.40
& $\mathbf{5.81(1.92)}$ & $\mathbf{6.77(0.48)}$ & $\mathbf{6.67(0.62)}$ 
& $\mathbf{6.26(0.77)}$ & $\mathbf{6.60(1.31)}$ & $7.32(0.30)$ \\
\midrule
\multirow{7}{*}{Subj}
& 0.10
& $6.23(1.08)$ & $1.65(0.52)$ & $0.79(0.38)$ 
& $\mathbf{0.00(0.00)}$ & $\mathbf{0.00(0.00)}$ & $6.03(0.54)$ \\
& 0.15
& $6.14(1.52)$ & $2.23(0.38)$ & $1.07(0.42)$ 
& $\mathbf{0.00(0.00)}$ & $\mathbf{0.00(0.00)}$ & $6.50(0.31)$ \\
& 0.20
& $6.65(1.60)$ & $2.75(0.45)$ & $1.46(0.32)$ 
& $0.97(0.48)$ & $\mathbf{0.00(0.00)}$ & $7.14(0.51)$ \\
& 0.25
& $7.70(1.20)$ & $3.33(0.46)$ & $2.18(0.48)$ 
& $1.77(0.27)$ & $\mathbf{0.00(0.00)}$ & $7.62(0.38)$ \\
& 0.30
& $6.08(1.07)$ & $3.52(0.39)$ & $3.02(0.28)$ 
& $3.22(0.35)$ & $\mathbf{2.15(0.96)}$ & $8.39(0.30)$ \\
& 0.35
& $7.50(1.13)$ & $\mathbf{4.50(0.42)}$ & $\mathbf{4.37(0.27)}$ 
& $4.63(0.34)$ & $5.11(0.30)$ & $9.02(0.31)$ \\
& 0.40
& $6.75(0.73)$ & $\mathbf{5.60(0.29)}$ & $6.70(0.30)$ 
& $7.16(0.41)$ & $7.33(0.31)$ & $9.74(0.25)$ \\
\midrule
\multirow{7}{*}{Twonorm}
& 0.10
& $\mathbf{0.12(0.22)}$ & $\mathbf{0.00(0.00)}$ & $\mathbf{0.00(0.00)}$ 
& $\mathbf{0.00(0.00)}$ & $\mathbf{0.00(0.00)}$ & $0.51(0.20)$ \\
& 0.15
& $0.39(0.24)$ & $\mathbf{0.00(0.00)}$ & $\mathbf{0.00(0.00)}$ 
& $\mathbf{0.00(0.00)}$ & $\mathbf{0.00(0.00)}$ & $0.80(0.15)$ \\
& 0.20
& $0.42(0.33)$ & $\mathbf{0.00(0.00)}$ & $\mathbf{0.00(0.00)}$ 
& $\mathbf{0.00(0.00)}$ & $\mathbf{0.00(0.00)}$ & $0.82(0.19)$ \\
& 0.25
& $0.44(0.30)$ & $\mathbf{0.01(0.02)}$ & $\mathbf{0.00(0.00)}$ 
& $\mathbf{0.00(0.00)}$ & $\mathbf{0.00(0.00)}$ & $1.02(0.11)$ \\
& 0.30
& $0.42(0.19)$ & $\mathbf{0.02(0.03)}$ & $\mathbf{0.00(0.01)}$ 
& $\mathbf{0.02(0.02)}$ & $0.09(0.07)$ & $1.03(0.11)$ \\
& 0.35
& $0.50(0.24)$ & $\mathbf{0.04(0.05)}$ & $\mathbf{0.04(0.03)}$ 
& $0.11(0.07)$ & $0.39(0.10)$ & $1.15(0.15)$ \\
& 0.40
& $0.71(0.39)$ & $\mathbf{0.09(0.04)}$ & $0.26(0.06)$ 
& $0.34(0.08)$ & $0.73(0.13)$ & $1.24(0.10)$ \\
\midrule
\multirow{7}{*}{MNIST}
& 0.10
& $2.37(0.10)$ & $\mathbf{0.05(0.04)}$ & $\mathbf{0.04(0.03)}$ 
& $0.08(0.03)$ & $0.18(0.03)$ & $0.55(0.51)$ \\
& 0.15
& $2.23(0.20)$ & $\mathbf{0.02(0.02)}$ & $0.09(0.02)$ 
& $0.29(0.06)$ & $0.32(0.03)$ & $0.58(0.15)$ \\
& 0.20
& $2.36(0.09)$ & $\mathbf{0.05(0.04)}$ & $0.17(0.03)$ 
& $0.43(0.05)$ & $0.40(0.05)$ & $0.55(0.12)$ \\
& 0.25
& $2.33(0.18)$ & $\mathbf{0.05(0.04)}$ & $0.34(0.05)$ 
& $0.54(0.05)$ & $0.45(0.04)$ & $0.50(0.09)$ \\
& 0.30
& $2.41(0.17)$ & $\mathbf{0.05(0.02)}$ & $0.55(0.06)$ 
& $0.60(0.06)$ & $0.48(0.07)$ & $0.52(0.10)$ \\
& 0.35
& $2.30(0.13)$ & $\mathbf{0.10(0.02)}$ & $0.87(0.09)$ 
& $0.61(0.07)$ & $0.48(0.08)$ & $0.52(0.11)$ \\
& 0.40
& $2.39(0.22)$ & $\mathbf{0.10(0.03)}$ & $1.17(0.10)$ 
& $0.52(0.06)$ & $0.46(0.03)$ & $0.53(0.08)$ \\
\midrule
\multirow{7}{*}{Fashion-MNIST}
& 0.10
& $11.47(0.21)$ & $\mathbf{1.86(0.44)}$ & $2.77(0.47)$ 
& $\mathbf{1.95(0.09)}$ & $2.78(0.15)$ & $\mathbf{1.06(1.59)}$ \\
& 0.15
& $11.49(0.40)$ & $\mathbf{1.93(0.49)}$ & $3.62(0.28)$ 
& $3.98(0.20)$ & $4.40(0.17)$ & $4.66(0.59)$ \\
& 0.20
& $11.77(0.30)$ & $\mathbf{2.17(0.36)}$ & $4.85(0.35)$ 
& $5.07(0.23)$ & $5.11(0.14)$ & $6.05(0.73)$ \\
& 0.25
& $11.56(0.46)$ & $\mathbf{2.06(0.33)}$ & $6.40(0.31)$ 
& $5.48(0.13)$ & $5.19(0.12)$ & $6.48(0.90)$ \\
& 0.30
& $11.68(0.37)$ & $\mathbf{2.45(0.39)}$ & $7.54(0.41)$ 
& $5.33(0.32)$ & $4.91(0.13)$ & $5.50(0.48)$ \\
& 0.35
& $11.60(0.31)$ & $\mathbf{2.85(0.45)}$ & $8.50(0.23)$ 
& $4.82(0.42)$ & $4.51(0.22)$ & $4.41(0.35)$ \\
& 0.40
& $11.63(0.31)$ & $\mathbf{2.96(0.52)}$ & $9.50(0.23)$ 
& $3.98(0.31)$ & $3.86(0.33)$ & $3.83(0.46)$ \\
\midrule
\multirow{7}{*}{KMNIST}
& 0.10
& $11.27(0.34)$ & $\mathbf{0.44(0.15)}$ & $0.70(0.19)$ 
& $0.58(0.13)$ & $0.89(0.09)$ & $2.74(3.11)$ \\
& 0.15
& $11.11(0.26)$ & $\mathbf{0.49(0.16)}$ & $1.16(0.24)$ 
& $1.42(0.20)$ & $1.66(0.14)$ & $3.17(0.74)$ \\
& 0.20
& $11.51(0.46)$ & $\mathbf{0.57(0.14)}$ & $1.74(0.24)$ 
& $2.43(0.20)$ & $2.41(0.14)$ & $3.46(0.18)$ \\
& 0.25
& $11.41(0.47)$ & $\mathbf{0.68(0.17)}$ & $2.81(0.35)$ 
& $3.19(0.24)$ & $2.85(0.18)$ & $3.87(0.53)$ \\
& 0.30
& $11.35(0.28)$ & $\mathbf{0.73(0.10)}$ & $3.88(0.22)$ 
& $4.06(0.23)$ & $3.29(0.21)$ & $3.45(0.25)$ \\
& 0.35
& $11.35(0.29)$ & $\mathbf{0.84(0.18)}$ & $5.87(0.36)$ 
& $4.62(0.24)$ & $3.56(0.18)$ & $3.77(0.31)$ \\
& 0.40
& $11.58(0.45)$ & $\mathbf{1.12(0.18)}$ & $7.25(0.33)$ 
& $4.60(0.25)$ & $3.47(0.14)$ & $3.86(0.23)$ \\
\bottomrule
\end{tabular}
} % \resizebox
\caption{Mean and standard error of $0\text{-}1$ risk for accepted data of the noisy-labeled setting (rescaled to $0-100$).}
\end{table*}

